Unsupervised Detection and Clustering of Malicious TLS Flows

Malware abuses TLS to encrypt its malicious traffic, preventing examination by content signatures and deep packet inspection. Network detection of malicious TLS flows is an important, but challenging, problem. Prior works have proposed supervised machine learning detectors using TLS features. However, by trying to represent all malicious traffic, supervised binary detectors produce models that are too loose, thus introducing errors. Furthermore, they do not distinguish flows generated by different malware. On the other hand, supervised multi-class detectors produce tighter models and can classify flows by malware family, but require family labels, which are not available for many samples. To address these limitations, this work proposes a novel unsupervised approach to detect and cluster malicious TLS flows. Our approach takes as input network traces from sandboxes. It clusters similar TLS flows using 90 features that capture properties of the TLS client, TLS server, certificate, and encrypted payload; and uses the clusters to build an unsupervised detector that can assign a malicious flow to the cluster it belongs to, or determine it is benign. We evaluate our approach using 972K traces from a commercial sandbox and 35M TLS flows from a research network. Our clustering shows very high precision and recall with an F1 score of 0.993. We compare our unsupervised detector with two state-of-the-art approaches, showing that it outperforms both. The false detection rate of our detector is 0.032% measured over four months of traffic.

==> Makefile <==
PROJECT=paper

# xfig documents whose corresponding EPS fies are used in the paper
# FIGFILES = segment.fig allocGroup.fig

# matlab scripts that generate output for the paper. These are *.m files
# that generate a corresponding *.eps file when run.
MFILES =

# GNUplot files
PLTFILES = 

# Other EPS files that are necessary to build the document
# If you have eps files that you generate by hand, list them here.
EPSFILES =

# Non-refdbms bib files to be included
# If you need a local .bib file, put that here.
LOCALBIB = bibliography/paper.bib
LOCALXTXBIB = bibliography/paper.xtx

# default targets to make for make all
TARGETS = $(PROJECT).pdf
TARGETSPS = $(PROJECT).ps

#-- Programs used when runing latex etc.                       
BIBTEX = bibtex
XTEX = crosstex
LATEX = latex
DVIPS = dvips -tletter
FIG2DEV = fig2dev
MATLAB = matlab
GNUPLOT = gnuplot
PS2PDF = ps2pdf
PDFLATEX = pdflatex

SRCFILES = $(wildcard *.tex)
EPSFIGFILES = $(FIGFILES:.fig=.eps)
EPSMFILES = $(MFILES:.m=.eps)
EPSPLTFILES = $(PLTFILES:.plt=.eps)
EPSFILES += $(EPSFIGFILES) $(EPSMFILES) $(EPSPLTFILES)

#--------------------------------------------------------------------------
# Production/target rules                       
#--------------------------------------------------------------------------
.SUFFIXES:
.PHONY: clean all veryclean
#-- EPS files may be expensive to regenerate, so keep them even though they
#-- are intermediate targets
.PRECIOUS: $(EPSMFILES) $(EPSFIGFILES)
#.PRECIOUS: $(EPSMFILES)

all: $(TARGETS)

#-- Make EPS files from matlab documents
%.eps: %.m
	$(MATLAB) -nodesktop -r "$*;quit" || $(MATLAB) -nodisplay -r "$*;quit"

#-- Make EPS files from xfig documents
%.eps: %.fig
	$(FIG2DEV) -L eps $< $@ || $(FIG2DEV) -L ps $< $@

#-- Make EPS files from GNUplot scripts
%.eps: %.plt
	$(GNUPLOT) $<

#-- Creation of initial .aux file
%.aux: %.tex $(SRCFILES) $(EPSFILES)
	$(LATEX) $<

#-- Create .bbl from .bib
%.bbl: %.aux $(LOCALBIB)
	$(BIBTEX) $*
	$(LATEX) $*.tex
	$(LATEX) $*.tex

#-- Build a dvi... 
#%.dvi: %.tex %.bbl $(EPSFILES) $(LOCALBIB)
%.dvi: %.tex %.bbl
	$(LATEX) $<

#-- converting .dvi to .ps... requires the EPS files
%.ps: %.dvi $(EPSFILES)
	$(DVIPS) -o $@ $<

#-- converting .ps to .pdf.
#%.pdf: %.ps
#	$(PS2PDF) $<

#-- generating pdf using pdflatex
%.pdf: %.tex $(SRCFILES) $(LOCALBIB)
	$(PDFLATEX) $*
#	$(BIBTEX) $*
#	$(PDFLATEX) $*
#	$(BIBTEX) $*
#	$(PDFLATEX) $*
	chmod +x $*.pdf

full: $(SRCFILES) $(LOCALBIB)
	$(PDFLATEX) $(PROJECT)
	$(BIBTEX) $(PROJECT)
	$(PDFLATEX) $(PROJECT)
	$(BIBTEX) $(PROJECT)
	$(PDFLATEX) $(PROJECT)
	chmod +x $(PROJECT).pdf
	

bib:	$(LOCALXTXBIB)
	$(XTEX) --short=state --short=conference --no-field editor --no-field publisher \
		--no-field pages --xtx2bib $(LOCALXTXBIB)

ps:	$(TARGETSPS)

pdf:
	$(PS2PDF) $(TARGETS)

clean:
	rm -f *~  $(TARGETS) $(TARGETSPS) *.dvi *.log *.aux *.blg *.bbl $(OLDAUX)

veryclean: clean
	rm -f $(EPSFIGFILES) $(EPSMFILES) $(EPSPLTFILES)

spell:	$(SRCFILES)
	detex $^ | spell | env LANG=C sort -u | env LANG=C comm -23 - ok-words

